Probing the validity of the diffuse mismatch model for phonons using atomistic simulations

Due to it's simplicity the diffuse mismatch model (DMM) remains a popular description of phonon transmission across solid-solid boundaries. However, it remains unclear in which situations the DMM should be expected to be a valid model of the underlying physics. Here, its validity is investigated mode-by-mode using a 3-dimensional extension of the frequency domain, perfectly matched layer (FD-PML) method, to study the interface between face-centered cubic solids with interdiffused atoms. While submonolayer levels of interdiffusion are found to increase the number of available modes for transmission, consistent qualitatively with the DMM, we do not find quantitative or qualitative convergence toward the DMM at higher levels of interdiffusion. In particular, contrary to the fundamental assumption of the DMM, modes are not found to lose memory of their initial polarization and wavevector. The transmission coefficients of randomly interdiffused and smoothly-graded interfaces are also compared. While smoothly graded interfaces show strong anti-reflection properties, selection rules still prohibit transmission of many modes, whereas interdiffused interfaces are not subject to such rules and achieve similar thermal interface conductance by transmitting with lower probability but using a wider range of modes.

==> Frequency_Decomposition.tex <==
Based on our analysis until now one question still remains; after the interaction of the phonon with the interface how is the scattered energy distributed in the Brillouin Zone. If the DMM is to be believed then the distribution of energy should be uniform on the iso-frequency surface. Previous, works have focused on modal decomposition of a wave packet after it has interacted with the interface primarily in one dimensional system [cite keblinski and some others]. While Gordiz et al. have calculated the modal contribution to thermal conductance for each mode on incident and transmission side in frequency space.

Here we obtain the modal decomposition of the scattered wave in k-space using a fast fourier transform (FFT) of the scattered wave. The fundamental requirement for commercial codes require the sampling rate be on a uniform grid. For an FCC lattice this poses to be a problem in cartesian space and thus this method requires us to work in a non-cartesian space where primitive vectors of the FCC lattice form our 3-Dimensional basis set given by $a_1= a/2 \hat{i}+ a/2 \hat{j}+ 0 \hat{k}, a_2= a/2 \hat{i}+ 0 \hat{j}+ a/2 \hat{k} & a_3= 0 \hat{i}+ a/2 \hat{j}+ a/2 \hat{k}$ where a is the lattice constant in of conventional lattice and $\hat{i}, \hat{j}, \hat{k}$ are unit vectors in cartesian space. Under this construct any atom is at a distance of $||a_n||$ in the n-th direction from another atom. Now let us describe the displacement of an atom located at $r= l\times a_1+m\times a_2+ n\times a3$ as $\tilde{u}(\tilde{r})$. Then fourier transform of $\tilde{u}$ along the three dimensions $a_n$ n= 1, 2, 3 is given by 

\begin{equation}
    \hat{u}(\tilde(k))= \int e^{-2\pi i \tilde{k}.\tilde{r}}\tilde{u}(\tilde{r})\bf{dr^3} 
    \label{eqn: Frequency_Decomp}
\end{equation}

Where \hat{u}(\tilde{k}) defines the amplitude of the wave with wave-vector $k= l'\times b_1+ m'\times b_2+ n'\times b_3$ where $b_1, b_2 & b_3$ are the reciprocal basis vectors. 
